Regression of Environmental Noise in LIGO Data

We address the problem of noise regression in the output of gravitational-wave (GW) interferometers, using data from the physical environmental monitors (PEM). The objective of the regression analysis is to predict environmental noise in the gravitational-wave channel from the PEM measurements. One of the most promising regression method is based on the construction of Wiener-Kolmogorov filters. Using this method, the seismic noise cancellation from the LIGO GW channel has already been performed. In the presented approach the Wiener-Kolmogorov method has been extended, incorporating banks of Wiener filters in the time-frequency domain, multi-channel analysis and regulation schemes, which greatly enhance the versatility of the regression analysis. Also we presents the first results on regression of the bi-coherent noise in the LIGO data.

==> bilinear.tex <==
\section{Bi-linear Noise}

Upconversion of noise when two source are involved is Bi-linear noise, which is based on the trigonametric identity
\begin{equation} \sin \theta \sin \varphi = \frac{1}{2}\cos(\theta - \varphi) - \frac{1}{2}\cos(\theta + \varphi), \end{equation}
the two signals $\sin (2 \pi f_1 t)$ and $\sin (2 \pi f_2 t)$ will combine to produce 
\begin{equation} \sin (2 \pi f_1 t)\sin (2 \pi f_2 t) = \frac{1}{2}\cos [2 \pi (f_1 - f_2) t] - \frac{1}{2}\cos [2 \pi (f_1 + f_2) t]. \label{upconversion} \end{equation}
If there are auxiliary channels measuring these two physical phenomenon, to achieve \ref{upconversion}, time series of these channels are multiplied to produce a witness channel.
